Combining Bayesian Optimization and Lipschitz Optimization

Bayesian optimization and Lipschitz optimization have developed alternative techniques for optimizing black-box functions. They each exploit a different form of prior about the function. In this work, we explore strategies to combine these techniques for better global optimization. In particular, we propose ways to use the Lipschitz continuity assumption within traditional BO algorithms, which we call Lipschitz Bayesian optimization (LBO). This approach does not increase the asymptotic runtime and in some cases drastically improves the performance (while in the worst-case the performance is similar). Indeed, in a particular setting, we prove that using the Lipschitz information yields the same or a better bound on the regret compared to using Bayesian optimization on its own. Moreover, we propose a simple heuristics to estimate the Lipschitz constant, and prove that a growing estimate of the Lipschitz constant is in some sense ``harmless''. Our experiments on 15 datasets with 4 acquisition functions show that in the worst case LBO performs similar to the underlying BO method while in some cases it performs substantially better. Thompson sampling in particular typically saw drastic improvements (as the Lipschitz information corrected for its well-known ``over-exploration'' phenomenon) and its LBO variant often outperformed other acquisition functions.

==> BO.tex <==
%!TEX root = ../main.tex
%\section{ Bayesian Optimization}
%In the context of these conflicting results, in this section we propose two strategies for improving the performance of Bayesian optimization methods. First, in the next section we introduce the concept of a``\safe" Bayesian optimization algorithm. This is an algorithm that does no worse than random in the worst case, but that might still take advantage of BO for functions with a high degree of smoothness. Second, since smooth functions are one class of function where BO has a large advantage over random, we propose to re-explore the idea of ``first-order" Bayesian optimization (FOBO) methods that use gradient information to improve performance. We show how gradient information can lead to improved performance, and also propose FOBO strategies that use directional derivatives. The advantage of using directional derivatives is that they reduce the cost and memory requirements of FOBO methods, while directional derivatives can be obtained by automatic differentiation for any analytic function (so can be used even in many "black box" situations where we don't have gradient code available).

%We consider the problem of minimizing a real-valued function $f$ over a domain $\mathcal{X}$ consisting of finite lower and upper bounds on every variable,
%\begin{equation}
%\argmin{x \in \mathcal{X}} f(x).
%\label{eq:global-opt}
%\end{equation}
%We first consider a zero-order oracle where on iteration $t$ the algorithm can learn about the function by choosing a parameter value $x^t$ and receiving the corresponding function value $f(x^t)$. In this model, we consider the goal of trying to minimize the number of iterations $t$ before we can guarantee that we find a parameter value $\hat{x}$ such that $f(\hat{x}) - f^* \leq \epsilon$ (where $f^*$ is the minimum of $f$ and $\epsilon$ is some positive constant). In this work we will primarily be interested in BO methods based on Gaussian processes. Algorithm~ \ref{alg:BO} gives pseudo-code for BO. We will consider deterministic functions, but we expect that these observations also hold in other settings.
%
%Firstly, we note that finding such an $\hat{x}$ is \emph{impossible in any finite number of oracle calls} unless we make assumptions about $f$. Because the real numbers are uncountable, for any deterministic algorithms we can construct a function that achieves an arbitrarily low function value at a parameter setting that the algorithm will never try (and similar arguments hold for stochastic algorithms). Thus, to say anything in this setting we need some sort of continuity assumptions about the function $f$.
%
%One of the most natural assumption about $f$ that we might make is that $f$ is Lipschitz-continuous, meaning that the amount that $f$ can change as we change $x$ is bounded by a constant times the change in $x$. Under this assumption, it is known that \emph{any} algorithm requires $\Omega{(1/\epsilon^d)}$ iterations to reach an accuracy of $\epsilon$~\citep[Theorem~1.1.2]{Nes04b}. Further, an $O(1/\epsilon^d)$ worst-case rate can be achieved by using a grid-based search~\citep[Corollary~1.1.1]{Nes04b} or in expectation simply by trying random values for the $x^t$ (because the probability that a random $x$ is an $\epsilon$-optimal solution under this assumption is  $\Omega(\epsilon^d)$). Thus, in some sense random search is an \emph{optimal} algorithm. Further, this $O(1/\epsilon^d)$ rate is faster than the best known rates for BO in many settings, in the sense that the exponent of $\epsilon$ for BO can be larger than $d$~\citep[Theorems~1-4]{bull2011convergence}.\footnote{We state results in terms in terms of the number of needed iterations, but we could equivalently state results in terms of the error after a fixed number of iterations. For example, if we require $O(1/\epsilon^d)$ iterations to reach an accuracy of $\epsilon$ then we can guarantee a sub-optimality of $O(1/t^{1/d})$ after $t$ iterations.}
%
%However, for functions with a sufficient amount of smoothness BO can beat random search. In particular, under additional assumptions and using $\nu$ as a measure of smoothness of $f$, Bull shows in a fascinating result that a variant of BO only requires $\tilde{O}(1/\epsilon^{d/\nu})$ iterations~\citep[Theorem~5]{bull2011convergence}. Thus, for ``nice" functions where $\nu$ is greater than 1 BO can be exponentially faster than random search. This  gives support for the empirical observation that in some settings BO soundly beats random search.
%
%%\subsubsection{Bayesian Optimization}
%
%Unfortunately, in the black-box setting we typically don't know $\nu$ and so we don't know if it is greater or less than $1$. This motivates us to consider ``\safe" BO.
%
%
%\subsubsection{Harmless  BO}
%%\begin{itemize}
%In~\citep{ahmed2016we}, we introduced the concept of  a ``\safe" BO algorithm as a BO method that requires at most $O(1/\epsilon^d)$ iterations to achieve an accuracy of $\epsilon$ on a Lipschitz-continuous function, and thus up to a constant factor performs as well as random search in the worst case.
%%\end{itemize}
%
%% We propose a harmless BO method that requires at most $O(1/\epsilon^d)$ iterations to achieve an accuracy of $\epsilon$ on a Lipschitz-continuous function, and thus up to a constant factor performs as well as random search in the worst case.
%
%
%It is quite simple to achieve a harmless BO method by combining an existing BO method with an existing harmless method like random search. We simply alternate between performing the iterations of the two algorithms. For example, if on odd iterations we evaluate a random $x^t$ and on even iterations we apply a BO method, this would constitute a harmless BO method. This is actually quite similar to the ``$\epsilon$-greedy" approach that Bull requires just for convergence of BO (and which is a common way to address exploration-exploitation issues). Further, if our BO method is the method analyzed by Bull, then this simple \safe~BO method achieves the best known rate of $\tilde{O}(1/\epsilon^{\min\{d,d/\nu\}})$. This assumes that the BO method ignores the random search iterations, but in practice we would likely do better by giving the BO method access to these iterates. Indeed, we conjecture that better \safe~methods are possible which \emph{locally} try to exploit smoothness in certain regions by adapting to the properties of the black-box function. Similarly,  it might be possible to improve the method by biasing the random samples away from the points sampled by the GP.
%
%%Another possible direction for better BO is 
%
%\begin{algorithm}[tb]
%	\caption{ Bayesian optimization}
%	\label{alg:BO}
%	\begin{algorithmic}
%		\STATE {\bfseries Input:} initial vector $x_0$, observation $y_0$, $D_0=(x_0,y_0)$.
%		\FOR{iteration $n=0,1,2,\dots,N$} 
%		\STATE select new $x_{n+1}$ by optimizing acquisition function $a$ \\
%		\begin{equation}
%		\label{eq:acquistion}
%		x_{n+1} = \argmax{x \in \mathcal{X}} a(x;D_n)
%		\end{equation}
%		\STATE query objective function to obtain $y_{n+1}$.
%		\STATE update model by $D_{n+1}=(x_{n+1}, y_{n+1})$ %$D_{n+1} = {D_{n},(x_{n+1}, y_{n+1})}$
%		%		\STATE $x_{0}$=$x^s$\\
%		%		\FOR{$t=1,2,\dots,m$} 
%		%		\STATE Randomly pick $i_{t} \in {1,\dots, n}$\\
%		%		\STATE $x_{t}=x_{t-1}-\eta(f_{i_{t}}^{'}(x_{t-1})-f_{i_{t}}^{'}(x^s)+\mu^s)\hfill(*)$\\
%		%		\ENDFOR
%		%		\STATE {\bfseries option I:} set $x^{s+1}=x_{m}$\\
%		%		\STATE {\bfseries option II:} set $x^{s+1}=x_{t}$ for random $t \in \{1,\dots, m\}$\\
%		\ENDFOR
%		\RETURN location of the maximum
%	\end{algorithmic}
%\end{algorithm}
%
%\subsubsection{First Order  BO}
%Making a BO method \safe~protects it from obtaining poor performance on functions with a low degree of smoothness, but often we are faced with minimizing a function with a high degree of smoothness. 

%In this differentiable case we should expect to improve performance by incorporating knowledge of the derivatives at the guesses $x^t$. We call methods based on this extra information first-order Bayesian optimization (FOBO) methods.
%
%Incorporating derivative observations in Gaussian processes is not a
%new idea~\citep{morris1993bayesian,solak:2003,Rasmussen:2006,Osborne:2010}, and there has been preliminary work on using derivative information specifically for the purpose of Bayesian optimization on two-dimensional
%problems~\citep[Section 5.2.4]{Lizotte:2008}. In this section, we revisit this idea in higher dimensions and also explore how directional derivatives can reduce the time/memory as well as the need to write gradient code when all that we have available is a zero-order black box.
%
%The usual BO assumption is that the values of $f$ are jointly Gaussian, being generated by a Gaussian process. We can incorporate derivative information by also assuming that derivatives are being generated by a Gaussian process.
%In particular, we'll assume that the
%function values and all first derivatives of~$f$ are jointly Gaussian and that the covariance kernel is twice differentiable.
%In this setting, the additional elements of the covariance kernel involving partial derivatives are given by~\citep{papoulis:2002,adler:2010}
%\begin{align}
%\mathrm{cov}(f(x^i), \partial_p f(x^j)) =
%\partial_p k(x^i,x^j),\ \text{and}
%\\
%\mathrm{cov}(\partial_p f(x^i), \partial_q f(x^j)) =
%\partial_p \partial_q k(x^i, x^j),
%\end{align}
%where $\partial_p f$ denotes the partial derivative of $f$ with respect to
%direction~$p$. Therefore, as long as the kernel is twice differentiable and the gradient can be
%evaluated, the GP can be extended to include gradient observations. Further, we conjecture that including gradient observations can further reduce the exponent in the iteration complexity of BO methods.
%%for convenience, we call this model GradGP.
%
%While the cost of computing gradients for analytic functions cannot be more than a constant factor more expensive than computing the function value, the memory and time requirement of the GP model increase if we use the full gradient of each $x^t$. In particular, the memory is increased from $O(t^2)$ to $O(t^2d^2)$ when we have $d$ variables. Similarly, the cost of the GP is increased from $O(t^3)$ to $O(t^3d^3)$ (assuming we use an exact solver, for illustration purposes). If this extra memory requirement is too large, then we propose to instead of modelling the gradient as a GP to instead model a \emph{directional derivative} $\partial_p f(x^t)$ for a particular direction $p$. The most logical direction $p$ to consider is the gradient direction, $\nabla f(x^t)$. This directional derivative still provides information about how the function changes, but since it is a scalar, it only increases the time/memory by a constant factor. 
%
%In many scenarios where BO is applied it is possible to compute gradients. For example, Bengio as well as Maclaurin et al.~have shown how to compute gradients with respect to hyper-parameters of machine learning models~\citep{bengio2000gradient,maclaurin2015gradient}. It is likely that these existing methods could be improved through the use of FOBO. On the other hand, sometimes we really have a ``black box" and cannot get access to the gradient. In these settings, as long as the function is analytic, it is always possible to use automatic differentiation to obtain directional derivatives $\partial_p f(x^t)$ for a given direction $p$ for a small increase in the cost of evaluating the black box. A particularly nice way of doing this is with the complex-step trick~\citep{martins2003complex}. Our experiments indicate that simply setting $p$ to a random direction can be more effective than standard BO methods for smooth functions.


==> theory.tex <==
%!TEX root = ../main.tex
\section{Theoretical analysis}

